Proving Equivalence Between Complex Expressions Using Graph-to-Sequence Neural Models

We target the problem of provably computing the equivalence between two complex expression trees. To this end, we formalize the problem of equivalence between two such programs as finding a set of semantics-preserving rewrite rules from one into the other, such that after the rewrite the two programs are structurally identical, and therefore trivially equivalent.We then develop a graph-to-sequence neural network system for program equivalence, trained to produce such rewrite sequences from a carefully crafted automatic example generation algorithm. We extensively evaluate our system on a rich multi-type linear algebra expression language, using arbitrary combinations of 100+ graph-rewriting axioms of equivalence. Our machine learning system guarantees correctness for all true negatives, and ensures 0 false positive by design. It outputs via inference a valid proof of equivalence for 93% of the 10,000 equivalent expression pairs isolated for testing, using up to 50-term expressions. In all cases, the validity of the sequence produced and therefore the provable assertion of program equivalence is always computable, in negligible time.

==> Makefile <==
FILENAME = cc21

ALLBIBS =					\
./lnp.bib					\
./images/lnp.bib				\
./pldi20.bib					\
./nips/paper/lnp.bib				\
./nips/paper/NeurIPS20.bib			\
./nips/paper/bibs/gabriel.bib			\
./nips/paper/bibs/refs.bib			\
./nips/paper/bibs/ierefs.bib			\
./nips/paper/bibs/lnp.bib			\
./nips/paper/bibs/lnp-bk.bib			\
./nips/paper/bibs/ics15.bib			\
./nips/paper/bibs/IMPACT18.bib			\
./nips/paper/bibs/popl.bib			\
./iclr/paper/ICLR21.bib				\
./iclr/paper/lnp.bib				\
./iclr/paper/iclrcc.bib				\
./iclr/paper/bibs/gabriel.bib			\
./iclr/paper/bibs/refs.bib			\
./iclr/paper/bibs/lnp.bib			\
./iclr/paper/bibs/lnp-bk.bib			\
./iclr/paper/bibs/ics15.bib			\
./iclr/paper/bibs/IMPACT18.bib			\
./iclr/paper/bibs/popl.bib			\
./bibs/cc21.bib					\
./bibs/gabriel.bib				\
./bibs/refs.bib					\
./bibs/ierefs.bib				\
./bibs/lnp.bib					\
./bibs/lnp-bk.bib				\
./bibs/ics15.bib				\
./bibs/IMPACT18.bib				\
./bibs/popl.bib


all:
	pdflatex $(FILENAME).tex
	bibtex $(FILENAME)
	pdflatex $(FILENAME).tex
	pdflatex $(FILENAME).tex

pdflatex:
	latex $(FILENAME).tex
	bibtex $(FILENAME)
	latex $(FILENAME).tex
	latex $(FILENAME).tex
	dvips -Ppdf $(FILENAME).dvi -o $(FILENAME).ps
	ps2pdf $(FILENAME).ps $(FILENAME).pdf

lnp:
	texi2pdf $(FILENAME).tex

clean:
	rm -f $(FILENAME).aux
	rm -f $(FILENAME).bbl
	rm -f $(FILENAME).blg
	rm -f $(FILENAME).log 
	rm -f $(FILENAME).ps
	rm -f $(FILENAME).dvi
	rm -f $(FILENAME).out

distclean: clean
	rm -f $(FILENAME).pdf
	rm -f $(FILENAME).out

pre-prepress:
	pdflatex $(FILENAME).tex
	pdflatex $(FILENAME).tex
	pdflatex $(FILENAME).tex

prepress: $(FILENAME).pdf
	ps2pdf14 -dPDFSETTINGS=/prepress $(FILENAME).pdf $(FILENAME)-prepress.pdf



bibcreate:
	bibtool -s -d -x $(FILENAME).aux $(ALLBIBS) > $(FILENAME).bib


==> images/tab-shape1.tex <==
\begin{tabular}{llrrrrrrrrrrr}
\toprule
       & benchmark &      2mm &      3mm &      adi &  cholesky &  doitgen &       lu &      mvt &  nussinov &  seidel-2d &  trisolv &     trmm \\
\midrule
cycles & gcc -O0 & 2.61e+10 &  4.4e+10 & 5.96e+10 &  1.45e+10 &  6.8e+09 &  5.1e+10 &  1.3e+08 &   5.1e+10 &   8.67e+10 & 2.04e+07 & 1.25e+10 \\
       & gcc -O1 & 1.52e+10 & 2.51e+10 & 4.17e+10 &   1.2e+10 & 4.53e+09 & 2.64e+10 & 9.72e+07 &  2.16e+10 &   8.57e+10 & 1.89e+07 & 9.38e+09 \\
       & gcc -O3 -novec & 7.24e+09 & 1.22e+10 & 3.33e+10 &  5.68e+09 & 2.08e+09 &  1.9e+10 & 7.81e+07 &  1.79e+10 &   7.58e+10 & 9.39e+06 & 8.39e+09 \\
       & gcc -O3 & 7.19e+09 & 1.21e+10 & 3.34e+10 &  5.69e+09 & 2.07e+09 & 1.81e+10 & 7.82e+07 &  1.78e+10 &   7.58e+10 & 9.37e+06 &  8.1e+09 \\
       & PyPy & 1.88e+10 & 3.07e+10 & 5.06e+10 &  1.27e+10 & 5.69e+09 & 3.66e+10 & 1.13e+08 &  5.81e+10 &    8.7e+10 & 2.47e+07 & 1.06e+10 \\
       & PyPy w/LE & 1.68e+10 & 2.62e+10 & 4.99e+10 &  8.94e+09 & 5.18e+09 & 3.52e+10 & 1.09e+08 &  5.31e+10 &        NaN & 2.04e+07 & 1.03e+10 \\
inst & gcc -O0 & 6.45e+10 & 1.03e+11 & 1.43e+11 &  5.07e+10 & 2.43e+10 & 1.01e+11 & 2.56e+08 &   1.2e+11 &   2.14e+11 & 6.41e+07 & 2.28e+10 \\
       & gcc -O1 & 1.41e+10 & 2.16e+10 & 2.89e+10 &  1.07e+10 & 4.35e+09 &  2.4e+10 &    6e+07 &  2.61e+10 &    2.8e+10 &  1.6e+07 & 4.81e+09 \\
       & gcc -O3 -novec & 1.16e+10 & 1.89e+10 & 1.89e+10 &  8.02e+09 & 3.81e+09 & 1.87e+10 &  5.2e+07 &  2.61e+10 &      3e+10 &  1.2e+07 & 4.21e+09 \\
       & gcc -O3 & 1.16e+10 & 1.89e+10 & 1.89e+10 &  8.02e+09 &  3.8e+09 & 1.87e+10 &  5.2e+07 &  2.61e+10 &      3e+10 &  1.2e+07 & 4.21e+09 \\
       & PyPy & 5.33e+10 & 8.43e+10 &  1.3e+11 &  3.91e+10 & 1.74e+10 & 8.34e+10 & 2.42e+08 &  1.21e+11 &   1.84e+11 & 8.26e+07 & 2.01e+10 \\
       & PyPy w/LE &    5e+10 & 7.89e+10 & 1.15e+11 &  3.64e+10 & 1.63e+10 & 7.82e+10 & 2.26e+08 &  1.02e+11 &        NaN & 5.86e+07 & 1.89e+10 \\
stalls & gcc -O0 & 3.02e+09 & 6.26e+09 & 4.78e+09 &   5.5e+08 & 1.33e+08 & 1.19e+10 & 3.14e+07 &  6.41e+09 &   8.49e+09 &  1.9e+06 & 2.51e+09 \\
       & gcc -O1 & 5.43e+09 & 1.04e+10 & 1.87e+10 &  4.14e+09 &  1.7e+09 & 1.15e+10 & 5.21e+07 &  6.21e+09 &    5.2e+10 & 7.08e+06 &    6e+09 \\
       & gcc -O3 -novec & 1.38e+09 & 3.67e+09 &  1.7e+10 &  2.19e+09 & 3.82e+08 & 1.02e+10 & 5.21e+07 &  7.15e+09 &   5.15e+10 & 4.14e+06 & 5.88e+09 \\
       & gcc -O3 &  1.6e+09 & 3.32e+09 &  1.7e+10 &  2.22e+09 & 4.63e+08 & 9.52e+09 & 5.21e+07 &  7.08e+09 &   5.15e+10 & 4.14e+06 &  5.6e+09 \\
       & PyPy & 5.24e+09 & 8.77e+09 & 1.91e+10 &  3.28e+09 & 1.15e+09 & 1.48e+10 & 5.52e+07 &  2.92e+10 &   4.11e+10 & 6.38e+06 & 5.47e+09 \\
       & PyPy w/LE & 5.25e+09 & 8.21e+09 & 2.24e+10 &  1.09e+09 & 1.36e+09 & 1.71e+10 & 6.42e+07 &  2.84e+10 &        NaN & 8.19e+06 & 5.85e+09 \\
l1m & gcc -O0 & 1.61e+09 & 2.67e+09 & 6.55e+08 &   9.6e+06 & 2.02e+08 & 2.47e+09 & 3.89e+06 &  2.33e+09 &   2.17e+07 & 1.25e+04 & 1.08e+09 \\
       & gcc -O1 & 1.63e+09 & 2.69e+09 & 6.25e+08 &  6.41e+06 & 3.71e+08 & 2.49e+09 & 3.94e+06 &  2.34e+09 &    1.2e+07 &    8e+03 & 1.09e+09 \\
       & gcc -O3 -novec & 1.63e+09 & 2.69e+09 & 6.36e+08 &  8.64e+06 & 4.91e+08 &  2.5e+09 & 3.95e+06 &  2.34e+09 &   1.17e+07 & 1.13e+04 & 1.08e+09 \\
       & gcc -O3 & 1.63e+09 & 2.69e+09 & 6.34e+08 &  8.68e+06 & 5.21e+08 &  2.5e+09 & 3.95e+06 &  2.34e+09 &   1.17e+07 & 1.11e+04 & 1.09e+09 \\
       & PyPy & 1.87e+09 & 3.25e+09 & 2.47e+09 &  1.82e+08 & 6.07e+08 & 3.22e+09 & 7.13e+06 &  3.56e+09 &    7.7e+08 & 3.05e+05 & 1.34e+09 \\
       & PyPy w/LE & 1.88e+09 &  3.3e+09 & 2.46e+09 &  1.81e+08 & 6.12e+08 & 3.26e+09 & 7.12e+06 &   3.5e+09 &        NaN & 3.02e+05 & 1.35e+09 \\
l2m & gcc -O0 & 3.92e+08 & 6.96e+08 & 3.73e+09 &  2.42e+08 & 9.13e+07 & 1.41e+09 & 6.89e+06 &  1.05e+09 &   3.36e+08 & 3.55e+05 & 4.22e+08 \\
       & gcc -O1 & 4.22e+08 & 7.02e+08 & 3.08e+09 &  2.42e+08 & 6.47e+07 & 1.27e+09 & 6.26e+06 &  1.05e+09 &   3.36e+08 & 3.55e+05 & 4.42e+08 \\
       & gcc -O3 -novec & 3.79e+08 & 6.76e+08 & 2.46e+09 &  2.42e+08 & 7.69e+07 & 1.27e+09 & 6.35e+06 &  1.07e+09 &   3.35e+08 & 3.55e+05 & 4.23e+08 \\
       & gcc -O3 & 4.04e+08 & 6.54e+08 & 2.45e+09 &  2.42e+08 & 6.57e+07 & 1.23e+09 & 6.48e+06 &  9.41e+08 &   3.35e+08 & 3.55e+05 & 4.71e+08 \\
       & PyPy &    6e+08 & 1.04e+09 & 4.61e+09 &  4.21e+08 &  1.5e+08 & 1.96e+09 & 1.03e+07 &  2.99e+09 &   5.77e+08 & 6.46e+05 & 6.71e+08 \\
       & PyPy w/LE & 5.72e+08 & 1.07e+09 & 4.47e+09 &  4.23e+08 & 1.31e+08 & 2.23e+09 &  9.8e+06 &  3.13e+09 &        NaN & 6.46e+05 &  6.6e+08 \\
l3m & gcc -O0 & 1.18e+07 & 3.03e+07 & 7.43e+08 &  6.01e+07 & 5.91e+05 & 1.36e+08 & 1.31e+06 &  2.13e+07 &   3.19e+08 & 4.21e+05 & 3.17e+06 \\
       & gcc -O1 & 9.33e+06 & 2.88e+07 & 7.17e+08 &  5.75e+07 & 5.87e+05 & 1.04e+08 & 1.25e+06 &  1.95e+07 &   2.94e+08 & 4.13e+05 &  2.6e+06 \\
       & gcc -O3 -novec & 7.99e+06 & 2.54e+07 & 7.17e+08 &  5.31e+07 & 5.51e+05 & 1.22e+08 & 1.22e+06 &  1.93e+07 &   2.91e+08 & 3.99e+05 & 2.72e+06 \\
       & gcc -O3 & 1.04e+07 & 2.51e+07 & 7.18e+08 &  5.47e+07 & 5.13e+05 & 1.13e+08 & 1.22e+06 &  1.86e+07 &   2.84e+08 & 3.86e+05 & 2.03e+06 \\
       & PyPy & 1.49e+07 & 4.12e+07 & 7.27e+08 &  6.49e+07 & 8.82e+05 &  1.6e+08 & 1.43e+06 &  2.56e+08 &   2.97e+08 &  4.1e+05 & 4.81e+06 \\
       & PyPy w/LE & 1.44e+07 & 3.65e+07 & 7.27e+08 &  6.29e+07 & 8.73e+05 & 1.82e+08 & 1.42e+06 &  2.51e+08 &        NaN & 4.09e+05 & 5.19e+06 \\
br & gcc -O0 & 1.66e+09 & 2.71e+09 &    2e+09 &  1.34e+09 & 5.51e+08 & 2.68e+09 & 8.01e+06 &  2.63e+09 &      2e+09 & 2.01e+06 & 6.03e+08 \\
       & gcc -O1 & 1.66e+09 &  2.7e+09 & 1.99e+09 &  1.34e+09 & 5.44e+08 & 2.67e+09 &    8e+06 &  2.62e+09 &      2e+09 &    2e+06 & 6.02e+08 \\
       & gcc -O3 -novec & 1.66e+09 &  2.7e+09 & 1.99e+09 &  1.34e+09 & 5.44e+08 & 2.67e+09 &    8e+06 &  2.61e+09 &      1e+09 &    2e+06 & 6.02e+08 \\
       & gcc -O3 & 1.66e+09 &  2.7e+09 & 1.99e+09 &  1.34e+09 & 5.42e+08 & 2.67e+09 &    8e+06 &  2.61e+09 &      1e+09 &    2e+06 & 6.02e+08 \\
       & PyPy & 1.33e+10 & 2.17e+10 &  3.4e+10 &  9.41e+09 & 4.47e+09 & 2.15e+10 & 5.22e+07 &  3.93e+10 &   5.59e+10 & 1.81e+07 & 5.45e+09 \\
       & PyPy w/LE & 1.33e+10 & 2.17e+10 &  2.9e+10 &  9.42e+09 & 4.47e+09 & 2.15e+10 & 5.22e+07 &  3.41e+10 &        NaN & 1.41e+07 & 5.46e+09 \\
brmissp & gcc -O0 & 1.68e+06 & 2.59e+06 &    2e+06 &  1.94e+06 & 3.42e+06 & 3.81e+06 & 4.01e+03 &  3.07e+06 &      1e+06 &    2e+03 & 1.14e+06 \\
       & gcc -O1 & 1.68e+06 & 2.59e+06 &    2e+06 &  1.96e+06 & 3.41e+06 & 3.84e+06 & 4.01e+03 &  3.06e+06 &      1e+06 & 1.98e+03 & 1.12e+06 \\
       & gcc -O3 -novec & 1.68e+06 & 2.59e+06 &    2e+06 &  1.95e+06 & 3.41e+06 & 3.82e+06 &    4e+03 &  3.07e+06 &   1.21e+06 & 1.99e+03 & 1.12e+06 \\
       & gcc -O3 & 1.68e+06 & 2.59e+06 &    2e+06 &  1.97e+06 & 3.41e+06 & 3.84e+06 & 4.00e+03 &  3.09e+06 &    1.2e+06 & 1.99e+03 & 1.12e+06 \\
       & PyPy &  1.7e+06 & 2.62e+06 &  2.2e+06 &  1.98e+06 & 3.41e+06 & 3.83e+06 & 4.44e+03 &  4.97e+06 &   1.03e+06 & 3.02e+03 & 1.12e+06 \\
       & PyPy w/LE &  1.7e+06 & 2.62e+06 & 2.05e+06 &  1.96e+06 & 3.43e+06 & 3.85e+06 & 4.34e+03 &   4.7e+06 &        NaN & 2.22e+03 & 1.11e+06 \\
loads & gcc -O0 & 3.06e+10 & 4.86e+10 & 6.68e+10 &   2.4e+10 &  9.2e+09 &  4.8e+10 &  1.2e+08 &  5.48e+10 &   8.58e+10 &    3e+07 & 1.08e+10 \\
       & gcc -O1 & 5.76e+09 &  8.1e+09 & 8.97e+09 &     4e+09 & 1.62e+09 &    8e+09 &  2.4e+07 &  7.83e+09 &      2e+10 &    6e+06 &  1.8e+09 \\
       & gcc -O3 -novec & 3.31e+09 &  5.4e+09 & 6.97e+09 &  2.67e+09 & 1.08e+09 & 5.34e+09 &  1.6e+07 &  5.22e+09 &   6.01e+09 &    4e+06 &  1.2e+09 \\
       & gcc -O3 & 3.31e+09 &  5.4e+09 & 6.97e+09 &  2.67e+09 & 1.08e+09 & 5.34e+09 &  1.6e+07 &  5.22e+09 &   6.01e+09 &    4e+06 &  1.2e+09 \\
       & PyPy & 8.41e+09 & 1.37e+10 & 2.16e+10 &  6.78e+09 & 2.92e+09 & 1.62e+10 & 4.03e+07 &  2.11e+10 &    3.6e+10 & 1.02e+07 & 3.68e+09 \\
       & PyPy w/LE & 6.75e+09 &  1.1e+10 & 1.86e+10 &  4.12e+09 & 2.39e+09 & 1.09e+10 & 2.83e+07 &  1.85e+10 &        NaN & 6.17e+06 & 3.08e+09 \\
stores & gcc -O0 & 3.32e+09 & 5.41e+09 & 4.99e+09 &  2.67e+09 & 1.09e+09 & 5.34e+09 &  1.6e+07 &  5.22e+09 &   3.99e+09 & 4.01e+06 &  1.2e+09 \\
       & gcc -O1 & 1.66e+09 &  2.7e+09 & 2.99e+09 &  1.34e+09 & 5.44e+08 & 2.67e+09 &    8e+06 &  2.61e+09 &      2e+09 &    2e+06 & 6.01e+08 \\
       & gcc -O3 -novec & 1.66e+09 &  2.7e+09 & 2.99e+09 &  1.34e+09 & 5.44e+08 & 2.67e+09 &    8e+06 &  2.61e+09 &      2e+09 &    2e+06 & 6.01e+08 \\
       & gcc -O3 & 1.66e+09 &  2.7e+09 & 2.99e+09 &  1.34e+09 & 5.42e+08 & 2.67e+09 &    8e+06 &  2.61e+09 &      2e+09 &    2e+06 & 6.01e+08 \\
       & PyPy & 6.69e+09 & 1.09e+10 & 1.25e+10 &  5.41e+09 & 2.31e+09 & 1.08e+10 & 3.22e+07 &  1.31e+10 &   8.02e+09 & 8.11e+06 & 2.45e+09 \\
       & PyPy w/LE & 5.03e+09 &  8.2e+09 &  1.3e+10 &  4.07e+09 & 1.76e+09 & 8.15e+09 & 2.42e+07 &  1.05e+10 &        NaN & 6.09e+06 & 1.85e+09 \\
\bottomrule
\end{tabular}


==> polybench.tex <==
%% {\color{red}

%% \begin{itemize}
%% \item GENERAL INTRODUCTION TO POLYBENCH (LN?).
%% \end{itemize}}

We now introduce PolyBench/Python, which is based on PolyBench/C, and
present the approach for the various kernel implementations we provide for each benchmark.


\subsection{PolyBench}



PolyBench is a benchmark suite of 30 numerical computations with
static control flow, extracted from operations in various application
domains (linear algebra computations, image processing, physics
simulation, dynamic programming, statistics, etc.). Its original
objective is to offer a set of representative numerical computations
that are amenable to polyhedral optimizations, and to offer a platform
to ease reproducibility of experiments, including numerous features
for e.g. cache flushing, highly accurate timing, support for PAPI
hardware counters, and non-random initialization data. PolyBench/C was
developed by Pouchet, with significant contributions from Yuki
starting PolyBench/C 4.0 \cite{polybench-url}.

PolyBench/Python is based on PolyBench/C 4.2.1 by Pouchet and
Yuki \cite{polybench-url}. By design, PolyBench/Python
implements \emph{exactly} the same computation as in the equivalent
PolyBench/C program: the same data types, exact same algorithm
(including the same execution order for the operations, for loop-based
Python implementations), and exact same dataset sizes. The objective
is to provide implementations in different languages of the exact same
computation to allow ``apple-to-apple'' comparisons between native C
implementations and JIT/interpreted implementations in Python, thereby
enabling to observe the overhead of the Python techniques compared to
the execution of only-necessary instructions in the native C program.

Table~\ref{table:polybenchdesc} presents the 30 kernels in PolyBench
and their description, for completeness. 


\begin{table}[h!tb]
\begin{center}
\caption{\label{table:polybenchdesc}30 kernels in PolyBench}
{\small
\begin{tabular}{l|l}


\textsf{Benchmark} &	\textsf{Description} \\ \hline
\texttt{2mm} &		2 Matrix Multiplications (alpha * A * B * C + beta * D) \\
\texttt{3mm} &		3 Matrix Multiplications ((A*B)*(C*D)) \\
\texttt{adi} &		Alternating Direction Implicit solver \\
\texttt{atax} &		Matrix Transpose and Vector Multiplication\\ 
\texttt{bicg} &		BiCG Sub Kernel of BiCGStab Linear Solver \\
\texttt{cholesky} &	Cholesky Decomposition \\
\texttt{correlation} &	Correlation Computation\\
\texttt{covariance} &	Covariance Computation\\
\texttt{deriche} &		Edge detection filter\\
\texttt{doitgen} &		Multi-resolution analysis kernel (MADNESS) \\
\texttt{durbin} &		Toeplitz system solver \\
\texttt{fdtd-2d} &		2-D Finite Different Time Domain Kernel\\
\texttt{gemm} &		Matrix-multiply C=alpha.A.B+beta.C\\
\texttt{gemver} &		Vector Multiplication and Matrix Addition\\
\texttt{gesummv} &		Scalar, Vector and Matrix Multiplication\\
\texttt{gramschmidt} &	Gram-Schmidt decomposition\\
\texttt{head-3d} &		Heat equation over 3D data domain\\
\texttt{jacobi-1D} &	1-D Jacobi stencil computation\\
\texttt{jacobi-2D} &	2-D Jacobi stencil computation\\
\texttt{lu} &		LU decomposition\\
\texttt{ludcmp} &		LU decomposition followed by Forward Substitution\\
\texttt{mvt} &		Matrix Vector Product and Transpose\\
\texttt{nussinov} &	Dynamic programming for sequence alignment\\
\texttt{seidel} &		2-D Seidel stencil computation\\
\texttt{symm} &		Symmetric matrix-multiply\\
\texttt{syr2k} &		Symmetric rank-2k update\\
\texttt{syrk} &		Symmetric rank-k update\\
\texttt{trisolv} &		Triangular solver\\
\texttt{trmm} &		Triangular matrix-multiply
\end{tabular}
}
\end{center}
\end{table}


\subsection{PolyBench/Python: General design}

The PolyBench/Python benchmarks have been implemented following the
Python 3 standard. Note no support was considered for Python 2 as it
was discontinued in early 2020~\cite{Python:Python2Discontinued}.

The actual benchmark implementation is built around
the \texttt{PolyBench} abstract class. It includes routines that
support benchmarking and array allocation, and defines abstract
handles that must be filled by implementing subclasses. In particular,
a benchmark will extend the \texttt{PolyBench} class and define the
abstract methods in
Figure~\ref{fig:PolyBench:AbstractFunctions}. These implement the
actual benchmark functionality, including array initialization, the
kernel code itself, and printing the results in a standardized format
which is readily compatible with the outputs produced by PolyBench/C,
allowing for cross-language validation. The \texttt{run\_benchmark()}
method is similar to \texttt{main()} in C codes. It is in charge of
defining the input and output structures of the benchmark, and
initializing them and running the kernel via calls to the appropriate
abstract methods.

\begin{figure}[h!tb]
\scriptsize
	\begin{verbatim}
def initialize_array(self, *args, **kwargs): ...
def print_array_custom(self, array: list, dump_message: str = ''): ...
def kernel(self, *args, **kwargs): ...
def run_benchmark(self) -> list[tuple]: ...
	\end{verbatim}
	\caption{Abstract functions to be implemented by a PolyBench/Python benchmark.}
	\label{fig:PolyBench:AbstractFunctions}
\end{figure}

PolyBench/Python provides two different ways to measure
performance. The first is to measure the execution time of the kernel
using the Timestamp Counter (TSC register). Its contents are directly
accessed using assembly code executed through the \texttt{inlineasm}
library. The second way is to measure performance counters using the
PAPI library~\cite{PAPIweb,PAPI} through the \texttt{python\_papi}
module.

\subsubsection{Implementations Available}

Translating PolyBench/C to Python requires a number of design
decisions to deal with the intrinsic differences between both
languages. One of the critical differences is related to data
representation. Polyhedral codes in general, and the PolyBench
benchmarks in particular, manipulate arrays and scalar variables of
basic types. In C, these are stored sequentially in memory in
row-major order. There is no equivalent representation in pure Python,
where everything is an object and there are no basic datatypes, in
contrast to other interpreted languages, such as Java, where both
concepts coexist. Since everything is an object, lists of \texttt{int}
values are not a collection of contiguously stored 32- or 64-bit basic
values, but rather a collection of contiguously stored 64-bit pointers
to \texttt{int} objects. This creates an additional level of
indirection which degrades performance when traversing the array.

Furthermore, when considering multidimensional structures, there is a
choice between implementing them as a sequence of nested lists,
similar to how a cascade of pointers to pointers would work in C, or
flattening the structure and linearizing the accesses, as
automatically done by C compilers with multidimensional array
allocations. One can envision how the flattening should be more
performant, in the same way that in C using cascaded pointers
introduces an additional level of indirection for each dimension in
the data structure, degrading memory performance.

One additional alternative for array implementation is to directly use
NumPy arrays~\cite{Python:NumPy}. This looks like a good design
alternative, since NumPy arrays are, by design, C-like objects, with
homogeneously-typed data and contiguous in memory. This has the
potential to greatly improve the memory behavior, and therefore
performance, but it comes with its own performance pitfalls that need
to be carefully studied.

In PolyBench/Python, the abstract \texttt{PolyBench} class that all
benchmarks must extend implements all these differents strategies for
array allocation. Figure~\ref{fig:PolyBench:ArrayImplementation}
details the three array implementation alternatives. The user must
select the desired implementation using runtime knobs. These
alternatives will be studied and compared in the experimental analysis
in Section~\ref{sec:expresults}.

\newsavebox{\gemmlist}
\begin{lrbox}{\gemmlist}
	\scriptsize
	\begin{minipage}{.49\columnwidth}
		\begin{verbatim}
for i in range(0, self.NI):
  for j in range(0, self.NJ):
    C[i][j] *= beta
  for k in range(0, self.NK):
    for j in range(0, self.NJ):
      C[i][j] += alpha * A[i][k] 
                       * B[k][j]
		\end{verbatim}
	\end{minipage}
\end{lrbox}%

\newsavebox{\gemmflist}
\begin{lrbox}{\gemmflist}
	\scriptsize
	\begin{minipage}{\columnwidth}
		\begin{verbatim}
for i in range(0, self.NI):
  for j in range(0, self.NJ):
    C[self.NJ * i + j] *= beta
  for k in range(0, self.NK):
    for j in range(0, self.NJ):
      C[self.NJ * i + j] += alpha * A[self.NK * i + k]
                                  * B[self.NJ * k + j]
		\end{verbatim}
	\end{minipage}
\end{lrbox}%

\newsavebox{\gemmnp}
\begin{lrbox}{\gemmnp}
	\scriptsize
	\begin{minipage}{.49\columnwidth}
		\begin{verbatim}
C *= beta
C += alpha * np.dot( A, B )
		\end{verbatim}
	\end{minipage}
\end{lrbox}%

\begin{figure}
	\subfloat[List]{\usebox{\gemmlist}}
	\subfloat[NumPy]{\usebox{\gemmnp}}\\
	\subfloat[Flattened List]{\usebox{\gemmflist}}
	\caption{List, flattened list, and NumPy alternative array implementations for the \texttt{gemm} kernel.}
	\label{fig:PolyBench:ArrayImplementation}
\end{figure}

\subsubsection{Control structures}

The PolyBench/C benchmark prominently feature two control
structures: \texttt{if} statements and \texttt{for} loops. The
conditionals have a direct translation to Python, with no semantic and
minimal syntactic variations. However, \texttt{for} loops in Python
are \emph{foreach} style loops that traverse a collection of
objects. In order to implement them efficiently a C \texttt{for} loop
is translated to a Python \texttt{for} traversing a \texttt{range}
expression. This is a special type of collection spawned by a
Python \texttt{generator} object. This kind of collections are
populated on demand, one object at a time, avoiding the memory
overhead of instantiating the full collection.


\subsection{Support for Polyhedral Optimizations}

We have implemented an
analysis and translation layer capable of reading Python kernels and
generating their ScopLib \cite{scoplib} representation, as
well as backgenerating Python codes from the ScopLib. The input to
this tool is not the Python source code, but the bytecode generated by
CPython. This allows the optimizations to be performed in a
just-in-time fashion, upon execution of the code, although this
approach has not been used in the current work. However, no search or
isolation of the static control part (SCoP) is performed at this
time. The tool receives a Python function and assumes its entire body
to be a valid SCoP.


\subsection{Python interpreters}

Similar as to using different compilers for C codes, a collection of
different interpreters exist for Python. CPython~\cite{Python:CPython}
is developed by the Python Software Foundation. Its goal is not to
achieve high performance, but to provide a multiplatform environment
that serves as the reference interpreter for other projects.

PyPy~\cite{Python:PyPy} is a performance-oriented interpreter
developed using the RPython~\cite{Ancona:RPython} toolchain. The
Python code is translated to RPython, which is then translated to flow
graphs, and then to C. The RPython layer includes a tracing
just-in-time layer including an optimizer and a back-end that
generates machine code.

Intel Distribution for Python~\cite{Python:IntelPython} is designed to
make Intel libraries such as the Math Kernel Library~\cite{Intel:MKL}
and the Data Analytics Acceleration Library~\cite{Intel:DAAL} usable
from Python. It does not intend to provide fast pure Python code, but
to bridge the technological gap between Python libraries such as NumPy
and Intel products.

The performance of these interpreters will be compared in the next section.


==> progequivstatic.tex <==
%% \section{Static Program Equivalence}
%% \label{sec:progequivstatic}
%% \input{progequivstatic}

%%%% LNP ===> FILE DELETED, instead use samplegen.tex.


%% \FIXME{LNP: This section will be totally revisited, to talk only about how to generate equivalent programs w/ steve's (simplified) random algo, and only briefly suggest how one can create a static brute-force checker. Will be done later}

%% Main idea: the brute-force program program equivalence algorithm that enumerates all possible rewrites is the one we make the neural net learn. input/output examples will be used for training, which are random path in the graph this algorithm explore. 


%% It is implicitly learning the algorithm used to generate examples, which is itself an algorithm that can explore the entire set of possible semantics-preserving tree rewrites. In essence, we make the neural network learn the acceleration heuristics to traversing such a space, but by using only classical input/output example-driven training.

%% maybe make a formal def for what is building a random valid path in the graph of transfo to generate program examples, to show it's the same formula for generating programs as it is to prove their equivalence from the previous section defs?


%% \subsection{Enumerating the Space of Equivalent Programs}


%% \subsection{Random Enumeration for Example Generation}

%% \FIXME{LNP: this is where your section currently in 5.1 will go, but I may take/split some parts and put them above. }


%% \subsection{Fast Equivalence Checking with Rewrite Rules}

%% pseudocode for applying the rewrite rule (while ensuring each rw is a valid axiom), and basic dfs-into-list + check lists are equal for the final structural equivalence check

